Deep Reinforcement Learning Control for Radar Detection and Tracking in Congested Spectral Environments

In this paper, dynamic non-cooperative coexistence between a cognitive pulsed radar and a nearby communications system is addressed by applying nonlinear value function approximation via deep reinforcement learning (Deep RL) to develop a policy for optimal radar performance. The radar learns to vary the bandwidth and center frequency of its linear frequency modulated (LFM) waveforms to mitigate mutual interference with other systems and improve target detection performance while also maintaining sufficient utilization of the available frequency bands required for a fine range resolution. We demonstrate that our approach, based on the Deep Q-Learning (DQL) algorithm, enhances important radar metrics, including SINR and bandwidth utilization, more effectively than policy iteration or sense-and-avoid (SAA) approaches in a variety of realistic coexistence environments. We also extend the DQL-based approach to incorporate Double Q-learning and a recurrent neural network to form a Double Deep Recurrent Q-Network (DDRQN). We demonstrate the DDRQN results in favorable performance and stability compared to DQL and policy iteration. Finally, we demonstrate the practicality of our proposed approach through a discussion of experiments performed on a software defined radar (SDRadar) prototype system. Our experimental results indicate that the proposed Deep RL approach significantly improves radar detection performance in congested spectral environments when compared to policy iteration and SAA.

==> bibb.tex <==
@misc{tensorflow,
    author    = "GoogleBrain",
    title     = "{TensorFlow}",
    url       = "https://www.tensorflow.org/"
}


@article{technical,
	author =       "Hugh Griffiths and Lawrence Cohen and Simon Watts and Eric Mokole and Chris Baker and Mike Wicks and Shannon Blunt",
	title =        "{Radar Spectrum Engineering and Management: Technical and Regulatory Issues}",
	journal =      "Proc. IEEE",
	volume =       "103",
	number =       "1",
	pages =        "85--102",
	year =         "Jan. 2015",
}

@article{xampling,
	author =       "Deborah Cohen and Kumar Vijay Mishra and Yonina C. Eldar",
	title =        "{Spectrum Sharing Radar: Coexistence via Xampling}",
	journal =      "IEEE Trans. Aerosp. Electron. Syst.",
	volume =       "54",
	number =       "3",
	pages =        "1279-1296",
	year =         "Dec. 2017",
}

@book{tse,
	author    = "David Tse and Pramod Viswanath",
	title     = "{Fundamentals of Wireless Communication}",
	year      = "2004",
	publisher = "Cambridge University Press",
}

@article{coexistence,
	author =       "Le Zheng and Marco Lops and Yonina C. Eldar and Xiaodong Wang",
	title =        "{Radar and Communication Co-existence: an Overview}",
	journal =      "IEEE Sig. Proc. Mag.",
	volume =       "36",
	number =       "5",
	pages =        "85-99",
	year =         "Sep. 2017",
}

@phdthesis{bell,
	author       = {Mark R. Bell}, 
	title        = {Information Theory and Radar: Mutual Information and the Design and Analysis of Radar Waveforms and Systems},
	school       = {California Institute of Technology},
	year         = 1988,
	address      = {},
	month        = 3,
	note         = {}
}

@book{handbook,
	author    = "Merrill I. Skolnik",
	title     = "{Radar Handbook}",
	year      = "2008",
	publisher = "McGraw-Hill",
}

@book{puterman,
	author    = "Martin L. Puterman",
	title     = "{Markov Decision Processes}",
	year      = "2005",
	publisher = "John Wiley and Sons Inc.",
}

@book{sutton,
	author    = "Richard S. Sutton and Andrew G. Barto",
	title     = "{Reinforcement Learning: An Introduction}",
	year      = "2018",
	publisher = "The MIT Press",
}

@article{natureDQN,
	author =       "Volodymyr Mnih and others",
	title =        "{Human-level control through deep reinforcement learning}",
	journal =      "Nature",
	volume =       "518",
	number =       "",
	pages =        "529-533",
	year =         "Feb. 2015",
}


@article{mlcomms,
	author =       "Osvaldo Simeone",
	title =        "{A Very Brief Introduction to Machine Learning With Applications to Communication Systems}",
	journal =      "IEEE Trans. Cog. Commun. and Netw.",
	volume =       "4",
	number =       "4",
	pages =        "648-662",
	year =         "Dec. 2018",
}

@article{ersin,
	author =       "Ersin Selvi and R. Michael Buehrer and Anthony Martone and Kelly Sherbondy",
	title =        "{Reinforcement Learning for Adaptable Bandwidth Tracking Radars}",
	journal =      "IEEE Trans. Aerosp. Electron. Syst.",
	volume =       "Early Access",
	number =       "",
	pages =        "",
	year =         "Apr. 2020"
}

@article{ontheroad,
	author =       "Maria S. Greco and Fulvio Gini and Pietro Stinco and Kristine Bell",
	title =        "{Cognitive Radars: On the Road to Reality Progress Thus Far and Possibilities for the Future}",
	journal =      "IEEE Sig. Proc. Mag.",
	volume =       "35",
	number =       "4",
	pages =        "112-125",
	year =         "July 2018",
}

@article{framework,
	author =       "Kristine L. Bell and Christopher J. Baker and Graeme E. Smith and Joel T. Johnson and Muralidhar Rangaswamy",
	title =        "{Cognitive Radar Framework for Target Detection and Tracking}",
	journal =      "IEEE J. of Sel. Topics in Sig. Proc.",
	volume =       "9",
	number =       "8",
	pages =        "1427-1438",
	year =         "Dec. 2015",
}


@article{dsa,
	author =       "Qing Zhao and Brian M. Sadler",
	title =        "{A Survey of Dynamic Spectrum Access}",
	journal =      "IEEE Sig. Proc. Mag.",
	volume =       "24",
	number =       "3",
	pages =        "79-89",
	year =         "May 2007",
}


@book{pomr,
	author    = "Mark A. Richards and James A. Cheer and William A. Holm",
	title     = "{Principles of Modern Radar: Basic principles}",
	year      = "2010",
	publisher = "Scitech Publishing",
}

@article{nimpc,
	author =       "Thomas Higgins and Karl Gerlach and Aaron K. Shackleford and Shannon D. Blunt",
	title =        "{Aspects of Non-Identical Multiple Pulse Compression}",
	journal =      "Proc. IEEE Radar Conf.",
	venue =        {Kansas City, MO},
	year =         {May 2011},
}

@article{richardson,
	author =       "Benjamin H. Kirk and Anthony F. Martone and Kelly D. Sherbondy and Ram M. Narayanan",
	title =        "{Mitigation of target distortion in pulse-agile sensors via Richardson–Lucy deconvolution}",
	journal =      "Electronics Letters",
	volume =       "55",
	number =       "23",
	pages =        "1249-1252",
	year =         "Nov 2019",
}

@article{multichanneldqn,
	author =       "Shangxing Wang and Hanpeng Liu and Pedro Henrique Gomes and Bhaskar Kishanamachari",
	title =        "{Deep Reinforcement Learning for Dynamic Multichannel Access in Wireless Networks}",
	journal =      "IEEE Transactions on Cognitive Communications and Networking",
	volume =       "4",
	number =       "2",
	pages =        "257-264",
	year =         "Jun. 2018",
}

@article{barto,
	author =       "Andrew G. Barto and Sridhar Mahadevan",
	title =        "{Recent Advances in Hierarchical Reinforcement Learning}",
	journal =      "Discrete Event Dynamic Systems",
	volume =       "13",
	number =       "",
	pages =        "41-77",
	year =         "Jan. 2003",
}

@article{arizona,
	author =       "Hamed Asadi and Haris Volos and Michael M. Marefat and Tamal Bose",
	title =        "{Metacognition and the Next Generattion of Cognitive Radio Engines}",
	journal =      "IEEE Communications Magazine",
	volume =       "54",
	number =       "1",
	pages =        "76-82",
	year =         "Jan. 2016",
}


@article{reed,
	author =       "Manik Gadhiok and Ashwin Amanna and Matthew J. Price and Jeffrey H. Reed",
	title =        "{Metacognition: Enhancing the performance of a cognitive radio}",
	journal =      "IEEE International Multi-Disciplinary Conference on Cognitive Methods in Situation Awareness and Decision Support",
	volume =       "",
	number =       "",
	pages =        "198-203",
	year =         "Feb. 2011",
}

@misc{deepcontext,
	author    = "Mark Collier and Hector U. Llorens",
	title     = "{Deep Contextual Multi-armed Bandits}",
	url       = "https://arxiv.org/abs/1807.09809"
}


@article{shirpa,
	author =       "Shirpa Agrawal and Navin Goyal",
	title =        "{Thompson Sampling for Contextual Bandits with Linear Payoffs}",
	journal =      "Proceedings of the 30th ICML",
	volume =       "",
	number =       "",
	pages =        "",
	year =         "Jun. 2013",
}

@article{empirical,
	author =       "Olivier Chapelle and Lihong Li",
	title =        "{An Empirical Evaluation of Thompson Sampling}",
	journal =      "Advances in Neural Information Processing Systems 24",
	volume =       "",
	number =       "",
	pages =        "2249-2257",
	year =         "Dec. 2011",
}

@article{mitola,
	author =       "Joesph Mitola and Gerald Q. Maguire",
	title =        "{Cognitive Radio: Making Software Radios More Personal}",
	journal =      "IEEE Personal Communications",
	volume =       "6",
	number =       "4",
	pages =        "13-18",
	year =         "Aug. 1999",
}

@article{haykin,
	author =       "Simon Haykin",
	title =        "{Cognitive Radar: a way of the future}",
	journal =      "IEEE Sig. Proc. Mag.",
	volume =       "23",
	number =       "1",
	pages =        "30-40",
	year =         "Jan. 2006",
}

@article{cogdynamic,
	author =       "Simon Haykin and Peyman Setoodeh and Shuo Fen and David Findlay",
	title =        "{Cognitive Dynamic System as the Brain of Complex Networks}",
	journal =      "IEEE J. on Sel. Areas of Commun.",
	volume =       "34",
	number =       "10",
	pages =        "2791-2799",
	year =         "Oct. 2016",
}

@book{esl,
	author    = "Trevor Hastie and Robert Tibshirani and Jerome Friedman",
	title     = "{The Elements of Statistical Learning: Data Mining, Inference, and Prediction}",
	year      = "2009",
	publisher = "Springer",
}

@misc{hajek,
	author    = "Bruce Hajek and Maxim Raginsky",
	title     = "{Statistical Learning Theory}",
	url       = "https://courses.grainger.illinois.edu/ece543/sp2019/SLT.pdf"
}


@article{hau92,
	author =       "David Haussler",
	title =        "{Decision Theoretic generalizations of the PAC model for neural net and other learning applications}",
	journal =      "Information and Computations",
	volume =       "95",
	number =       "",
	pages =        "129-161",
	year =         "Mar. 1992",
}

@book{bellman,
	author    = "Richard Bellman",
	title     = "{Adaptive Control Processes: A Guided Tour}",
	year      = "1961",
	publisher = "Princeton University Press",
}

@book{slivkins,
	author    = "Aleksandrs Slivkins",
	title     = "{Introduction to Multi-Armed Bandits}",
	year      = "2019",
	publisher = "Now Publishers",
}

@article{policysearch,
	author =       "J. Andrew Bagnell and Jeff Schneider",
	title =        "{Covariant Policy Search}",
	journal =      "Proceedings of the International Joint Conference on Artificial Intelligence",
	volume =       "",
	number =       "",
	pages =        "1019-1024",
	year =         "Aug. 2003",
}

@article{adam,
	author =       "Diederik P. Kingma and Jimmy Ba",
	title =        "{Adam: A Method for Stochastic Optimization}",
	journal =      "Proc. Intl. Conf. on Learn Rep. (ICLR)",
	volume =       "",
	number =       "",
	pages =        "1-15",
	year =         "May 2015",
}

@article{deeprlsurvey,
	author =       "Kai Arulkumaran and Marc Peter Deisenroth and Miles Brundage and Anil Anthony Bharath",
	title =        "{Deep Reinforcement Learning: A Brief Survey}",
	journal =      "IEEE Sig. Proc. Mag.",
	volume =       "34",
	number =       "6",
	pages =        "26-38",
	year =         "Nov. 2017",
}

@article{medicalCog,
	author =       "Cumhur Tas and Elliot C. Brown and Aysen Esen-Danaci and Paul H. Lysaker and Martin Brune",
	title =        "{Intrinsic motivation and metacognition as predictors of learning potential in patients with remitted schizophrenia}",
	journal =      "Journal of Pyschiatric Research",
	volume =       "46",
	number =       "8",
	pages =        "1086-1092",
	year =         "Aug. 2012",
}

@article{Ng,
	author =       "Andrew Y. Ng and Stuart J. Russel",
	title =        "{Algorithms for Inverse Reinforcement Learning}",
	journal =      "Proc. Intl. Conf. on Mach. Learn. (ICML)",
	volume =       "",
	number =       "",
	pages =        "663-670",
	year =         "Jul. 2000",
}

@article{ddql,
	author =       "Hado van Hassel and Arthur Guez and David Silver",
	title =        "{Deep Reinforcement Learning with Double Q-Learning}",
	journal =      "Proc. Conf. on Artificial Intelligence (AAAI)",
	volume =       "",
	number =       "",
	pages =        "2094-2099",
	year =         "Feb. 2016",
}

@article{lstm,
	author =       "Sepp Hochreiter and Jurgen Schmidhuber",
	title =        "{Long Short-Term Memory}",
	journal =      "Neural Computation",
	volume =       "9",
	number =       "8",
	pages =        "2094-2099",
	year =         "Nov. 1997",
}

@book{goodfellow,
	author    = "Ian Goodfellow and Yoshua Bengio and Aaron Courville",
	title     = "{Deep Learning}",
	year      = "2015",
	publisher = "The MIT Press",
}


@article{drql,
	author =       "Matthew Hausknecht and Peter Stone",
	title =        "{Deep Recurrent Q-Learning for Partially Observable MDPs}",
	journal =      "AAAI Fall Symposium Series",
	volume =       "9",
	number =       "8",
	pages =        "29-36",
	year =         "Sep. 2015",
}

@article{reconstruction,
	author =       "Ying-Hui Quan and others",
	title =        "{Range-Doppler reconstruction for frequency agile and PRF-jittering Radar}",
	journal =      "IET Radar Sonar, and Navigation",
	volume =       "12",
	number =       "3",
	pages =        "348-352",
	year =         "Jan. 2018",
}

@article{thompson,
author =       "William R. Thompson",
title =        "{On the Likelihood that One Unknown Probability Exceeds Another In View of The Evidence of Two Samples}",
journal =      "Biometrika",
volume =       "25",
number =       "3",
pages =        "285-294",
year =         "Dec. 1933",
}

@article{coopcb,
	author =       "Cem Tekin and Mihaela van der Schaar",
	title =        "{Distributed Online Learning via Cooperative Contextual Bandits}",
	journal =      "IEEE Transactions on Signal Processing",
	volume =       "63",
	number =       "14",
	pages =        "3700-3714",
	year =         "Jul. 2015",
}

@article{howmuch,
	author =       "Fan Liu and Adrian Garcia-Rodriguez and Christos Masouros and Giovanni Geraci",
	title =        "{Interfering Channel Estimation in Radar-Cellular Coexistence: How Much Information Do We Need?}",
	journal =      "IEEE Trans. Wireless Commun.",
	volume =       "18",
	number =       "9",
	pages =        "4238-4252",
	year =         "Sep. 2019",
}

@article{raghu,
	author =       "Raghunandan M. Rao and Harpreet S. Dhillon and Vuk Marojevic and Jeffrey H. Reed",
	title =        "{Analysis of Worst-Case Interference in Underlay Radar-Massive MIMO Spectrum Sharing Scenarios}",
	journal =      "{Proc. IEEE GLOBECOM}",
	volume =       "",
	number =       "",
	pages =        "",
	year =         "Dec. 2019",
}

@article{markovgame,
	author =       "Michael L. Littman",
	title =        "{Markov games as a framework for multi-agent reinforcement learning}",
	journal =      "Proc. Intl. Conf. on Mach. Learn. (ICML)",
	volume =       "",
	number =       "",
	pages =        "157-163",
	year =         "Jul. 1994",
}

@article{gui,
	author =       "Ronghua Gui and Wen-Quin Wang and Ye Pan and Jian Xu",
	title =        "{Cognitive Target Tracking via Angle-Range-Doppler Estimation with Transmit Subaperturing FDA Radar}",
	journal =      "IEEE J. of Sel. Topics in Sig. Proc.",
	volume =       "12",
	number =       "1",
	pages =        "76-89",
	year =         "Feb. 2018",
}

@article{cogbeamforming,
	author =       "Nathan Sharaga and Joesph Tabrikian and Hagit Messer",
	title =        "{Optimal Cognitive Beamforming for Target Tracking in MIMO Radar/Sonar}",
	journal =      "IEEE J. Sel. Topics in Sig. Proc.",
	volume =       "9",
	number =       "8",
	pages =        "1440-1451",
	year =         "Dec. 2015",
}

@article{multitrack,
	author =       "Li Wang and others",
	title =        "{Multi-Target Detection and Adaptive Waveform Design for Cognitive MIMO Radar}",
	journal =      "IEEE Sensors Journal",
	volume =       "18",
	number =       "24",
	pages =        "9962-9970",
	year =         "Dec. 2018",
}

@article{beamsharing,
	author =       "Zhe Geng and Hai Deng and Braham Himed",
	title =        "{Adaptive Radar Beamforming for Interference Mitigation in Radar-Wireless Spectrum Sharing}",
	journal =      "IEEE Sig. Proc. Letters",
	volume =       "22",
	number =       "4",
	pages =        "484-488",
	year =         "Apr. 2015",
}

@article{cognotch,
	author =       "Brandon Ravenscroft and others",
	title =        "{Experimental Demonstration and Analysis of Cognitive Spectrum Sensing and Notching for Radar}",
	journal =      "IET Radar, Sonar, and Nav.",
	volume =       "12",
	number =       "12",
	pages =        "1466-1475",
	year =         "Oct. 2018",
}

@article{infoMIMO,
	author =       "SaiDhiraj Amuru and R. Michael Buehrer and Ravi Tandon and Shabnam Sodagari",
	title =        "{MIMO Radar Waveform Design to support Spectrum Sharing}",
	journal =      "Military Communications Conference (MILCOM)",
	volume =       "",
	number =       "",
	pages =        "1535-1540",
	year =         "Nov. 2013",
}

@article{SDradar,
	author =       "Benjamin H. Kirk and others",
	title =        "{Avoidance of Time-Varying Radio Frequency Interference With Software-Defined Cognitive Radar}",
	journal =      "IEEE Trans. Aerosp. Electron. Syst.",
	volume =       "55",
	number =       "3",
	pages =        "1090-1104",
	year =         "Dec. 2018",
}

@article{kovarsky,
	author =       "Jacob A. Kovarskiy and Ram N. Narayanan and Anthony F. Martone and Kelly D. Sherbondy",
	title =        "{A Stochastic Model for Prediction and Avoidance of RF Interference to Cognitive Radars}",
	journal =      "Proc. IEEE Radar Conf.",
	volume =       "",
	number =       "",
	pages =        "",
	year =         "Apr. 2019",
}

@article{kozy,
	author =       "Mark Kozy and Jianyuan Yu and R. Michael Bueher and Anthony Martone and Kelly Sherbondy",
	title =        "{Applying Deep-Q Networks to Target Tracking to Improve Cognitive Radar}",
	journal =      "Proc. IEEE Radar Conf.",
	volume =       "",
	number =       "",
	pages =        "",
	year =         "Apr. 2019",
}

@article{factsheet,
	author =       "{Federal Communications Commission (FCC)}",
	title =        "{Spectrum Horizons}",
	journal =      "Fed. Registrar",
	volume =       "84",
	number =       "107",
	year =         "Jun. 2019",
}

@article{release,
	author =       "{Third Generation Partnership Project (3GPP)}",
	title =        "{5G in Release 17 - Strong Radio Evolution}",
	url   =        "",
	year =         "White Paper",
}

@article{yue,
	author =       "Yue Xu and Jet Yu and R. Michael Buehrer",
	title =        "{The Application of Deep Reinforcement Learning to Distributed Spectrum Access in Dynamic Heterogeneous Environments with Partial Observations}",
	journal =      "IEEE Trans. Wireless Commun.",
	volume =       "",
	number =       "",
	year =         "2020",
}

@article{key,
	author =       "{Keysight Technologies}",
	title =        "{Signal Studio for LTE/LTE-Advanced/LTE-Advanced Pro FDD/TDD}",
	url   =        "https://www.keysight.com/us/en/assets/7018-02606/technical-overviews/5990-6086.pdf",
	year =         "White Paper",
}

@article{demystified,
	author =       "Anthony F. Martone",
	title =        "Cognitive Radar Demystified",
	journal =      "USRI Bulletin",
	volume =       "",
	number =       "350",
	pages =        "10-22",
	year =         "2014",
}

@article{noncoop,
	author =       "Anthony F. Martone and Kenneth I. Ranney and Kelly Sherbondy and Kyle A. Gallagher and Shannon D. Blunt",
	title =        "{Spectrum Allocation for Noncooperative Radar Coexistence}",
	journal =      "IEEE Trans. Aerosp. Electron. Syst.",
	volume =       "54",
	number =       "1",
	pages =        "90-105",
	year =         "Aug. 2017",
}

@article{waveformopt,
	author =       "Bo Jiu and others",
	title =        "{Wideband cognitive radar waveform optimization for joint target radar signature estimation and target detection}",
	journal =      "IEEE Trans. Aerosp. and Elec. Sys.",
	volume =       "51",
	number =       "2",
	pages =        "1530-1546",
	year =         "Jun. 2017",
}

@book{resource,
	author    = "Peter Moo and Zhen Ding",
	title     = "{Adaptive Radar Resource Management}",
	year      = "2015",
	publisher = "Academic Press",
}

@article{isar,
	author =       "Joyanto Mukerjee and Paul Sheehan and Terrence Caelli",
	title =        "{Investigating Human Machine Integration Concepts for Isar Classification}",
	journal =      "Proc. Int. Commun., Nav. and Surv. Conf. (ICNS)",
	volume =       "",
	number =       "",
	pages =        "",
	year =         "Jun. 2019",
}

@article{radarcomms,
	author =       "Alex R. Chiriyath and Bryan Paul and Daniel W. Bliss",
	title =        "{Radar-Communications Convergence: Coexistence, Cooperation, and Co-Design}",
	journal =      "IEEE Trans. on Cogn. Commun. and Netw.",
	volume =       "3",
	number =       "1",
	pages =        "1-12",
	year =         "Mar. 2017",
}

@article{joint,
	author =       "{C. Sturm, T. Zwick, and W. Wiesbeck}",
	title =        "{An OFDM System Concept for Joint Radar and Communications Operations}",
	journal =      "Proc IEEE Vehic. Tech. Conf.",
	volume =       "",
	number =       "",
	pages =        "",
	year =         "Jun. 2009",
}

@book{intf,
	author    = "Martin Haenggi and Radha Krishna Ganti",
	title     = "{Interference in Large Wireless Networks}",
	year      = "2009",
	publisher = "Now Publishers",
}

@article{stinco,
	author =       "{P. Stinco, F. Gini and M. Greco}",
	title =        "{Spectrum sensing and sharing for cognitive radars}",
	journal =      "IET Radar, Sonar and Nav.",
	volume =       "10",
	number =       "3",
	pages =        "595-602",
	year =         "Feb. 2016",
}

@article{detection,
	author =       "{J. Metcalf, S.D. Blunt, and B. Himed}",
	title =        "{A Machine Learning Approach to Cognitive Radar Detection}",
	journal =      "Proc. IEEE Radar Conf.",
	volume =       "",
	number =       "",
	pages =        "1405-1411",
	year =         "Apr. 2015",
}

@article{pac,
	author =       "{V. Cutsuridis}",
	title =        "{Cognitive models of the perception-action cycle: A view from the brain}",
	journal =      "Proc. Intl. Joint Conf. on Neur. Netw.",
	volume =       "",
	number =       "",
	pages =        "",
	year =         "Aug. 2013",
}

@article{game,
	author =       "{Z. Ji and K. Liu}",
	title =        "{Cognitive Radios for Dynamic Spectrum Access - Dynamic Spectrum Sharing: A Game Theoretical Overview}",
	journal =      "IEEE Comm. Mag.",
	volume =       "45",
	number =       "5",
	pages =        "88-94",
	year =         "May 2007",
}

@article{multinn,
	author =       "{V. Schmidlin, G. Favier and R. Féraudt}",
	title =        "{Multitarget Radar Tracking with Neural Networks}",
	journal =      "Proc. IFAC Symp. on System Ident.",
	volume =       "27",
	number =       "8",
	pages =        "621-626",
	year =         "July 1994",
}

@article{tracknn,
	author =       "{A. N. Pineda \textit{et al.}}",
	title =        "{Radar Tracking System Using Contextual Information on a Neural Network Architecture in Air Combat Maneuvering}",
	journal =      "Intl. Jour. of Distributed Sensor Netw.",
	volume =       "9",
	number =       "8",
	pages =        "",
	year =         "Aug. 2013",
}

@article{wang,
	author =       "{J. Wang \textit{et al.}}",
	title =        "{Network Association in Machine-Learning Aided Cognitive Radar and Communication Co-Design}",
	journal =      "IEEE J. Sel. Areas in Commun.",
	volume =       "37",
	number =       "10",
	pages =        "",
	year =         "Oct. 2019",
}

@article{nulls,
	author =       "K. Gerlach and others",
	title =        "{Spectral Nulling on Transmit via Nonlinear FM Radar Waveforms}",
	journal =      "IEEE Trans. Aerosp. Electron. Syst.",
	volume =       "47",
	number =       "2",
	pages =        "1507-1515",
	year =         "Apr. 2011",
}

@article{metacog,
	author =       "Anthony F. Martone and others",
	title =        "{Metacognition for Radar Coexistence}",
	journal =      "Proc. IEEE Intl. Radar Conf.",
	volume =       "",
	number =       "",
	pages =        "",
	year =         "Apr. 2020",
}

@article{understanding,
	author =       "Zhuoran Yang and Yuchen Xie and Zhaoran Wang",
	title =        "{A Theoretical Analysis of Deep Q-Learning}",
	url =          "{https://arxiv.org/abs/1901.00137}"
	year =         "May 2019",
}

